TRAQ: Trustworthy Retrieval Augmented Question Answering via Conformal Prediction

When applied to open-domain question answering, large language models (LLMs) frequently generate incorrect responses based on made-up facts, which are called $\textit{hallucinations}$. Retrieval augmented generation (RAG) is a promising strategy to avoid hallucinations, but it does not provide guarantees on its correctness. To address this challenge, we propose the Trustworthy Retrieval Augmented Question Answering, or $\textit{TRAQ}$, which provides the first end-to-end statistical correctness guarantee for RAG. TRAQ uses conformal prediction, a statistical technique for constructing prediction sets that are guaranteed to contain the semantically correct response with high probability. Additionally, TRAQ leverages Bayesian optimization to minimize the size of the constructed sets. In an extensive experimental evaluation, we demonstrate that TRAQ provides the desired correctness guarantee while reducing prediction set size by 16.2% on average compared to an ablation. The implementation is available at $\href{https://github.com/shuoli90/TRAQ.git}{TRAQ}$.

==> sections/abstract.tex <==
\begin{abstract}
This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences. 
The document itself conforms to its own specifications, and is therefore an example of what your manuscript should look like.
These instructions should be used both for papers submitted for review and for final versions of accepted papers.
\end{abstract}

==> sections/introduction.tex <==
\section{Introduction}

% \begin{enumerate}
%     \item LLMs are powerful; but make hallucinations
%     \item RAG is an effective way to reduce hallucinations; but current RAG systems cannot guarantee their performance.
%     \item Conformal prediction is useful; but existing methods focus on the LLMs and also only on token-level confidence. (example)
%     \item Desiderata for trustworthy RAG:
%         \begin{itemize}
%             \item flexible with the retriever and generator
%             \item flexible with the API access (e.g., opensource vs black-box)
%             \item provide guarantee on the semantic level. (example)
%             \item Obtain small average prediction set size
%         \end{itemize}
%     \item Briefly describe our method
%     \item Our contributions:
%     \begin{itemize}
%         \item First one to provide guarantees for RAG systems
%         \item Satisfy the desirata
%         \item comprehensive experiments
%         \begin{itemize}
%             \item coverage levels; different random seeds
%             \item one fine-tuned dpr on medical datasets
%             \item four datasets
%             \item two LLMs(black-box and opensource)
%             \item different prompts
%             \item quantitative and qualitative results
%         \end{itemize}
%     \end{itemize}
% \end{enumerate}

Large language models (LLMs) have demonstrated state-of-the-art performance in many question answering (QA) tasks~\cite{openai2023gpt4, touvron2023llama, touvron2023llama2}. However, in open-domain QA tasks where candidate answers are not given, LLMs might confidently generate incorrect responses. These wrong responses are often called \textit{hallucinations}~\cite{ouyang2022training, kuhn2023semantic}. Hallucinations could induce catastrophic consequences if users incorporate them in making decisions, such as diagnosing a disease. Therefore, reducing hallucinations has attracted great interest, not only from the academia, but also from the public.

To reduce hallucinations, retrieval augmented generation (RAG)~\cite{lewis2021retrievalaugmented} has been shown to be effective. RAG consists of two steps, namely the \textit{retrieval step} and \textit{generation} step. In the retrieval step, given a query, RAG retrieves passages, e.g., Wikipedia paragraphs, from a knowledge corpus; in the generation step, RAG prompts an LLM with both the query and the retrieved passages. If the retrieved passages are relevant to the query, the LLM is likely to utilize related information to generate correct responses. \textbf{However, current RAG systems cannot guarantee its performance.} Specifically, in the retrieval step, relevant passages might not be submitted to the LLM. In this case, the LLM cannot obtain any useful information to reduce hallucinations. \unsure{In the generation step, the LLM cannot guarantee the rate that correct responses are generated, even after numerous responses are generated.} Though RAG achieves promising performance, these missing provable guarantees are indispensible in safety-critical domains like healthcare.

To obtain provable guarantees for RAG, \textit{conformal prediction}~\cite{shafer2007tutorial, angelopoulos2022gentle, park2020pac} is promising. Conformal prediction is a distribution-free uncertainty quantification technique. Given a machine learning model, conformal prediction post-process the predictions from the model to construct a set of labels, which guarantees to contain the true label with high probability. 

However, applying conformal prediction to RAG is non-trivial, especially for open-domain QA tasks. First, existing conformal prediction techniques require a finite label space like the finite categories in multi-class classification tasks. However, in the open-domain QA tasks, the label spaces, which are the collections of correct responses for different queries, are mostly infinite. Even for the same query, the correct response might be expressed in different ways in natural language. Second, existing conformal prediction on language modeling focus solely on the LLMs, instead of systems with multiple components like RAG. As demonstrated in our experiments, by applying conformal prediction and Bayesian optimization to the entire RAG pipeline, end-to-end efficiency can be improved by \todo{add quantitative results}, compared to treating individual components separately. Such efficiency should be any user-specified objectives, like the average number of semantic meanings in the constructed set. Third, existing techniques rely on predicted probabilities on individual outputs. If the underlying models are LLMs, these individual outputs are tokens or responses. \unsure{However, in open-domain QA tasks, different responses with the same semantic meaning should be regarded as the same}. For example, for the responses \textit{the capital of France is Paris} and \textit{Paris is the capital of France}, although they may have different predicted probabilities, they express the same semantic meaning and should be treated as the same. Furthermore, for some APIs such as \textit{gpt3.5-turbo}, the predicted probabilities for individual tokens or responses are not even accessible.

Given the limitations mentioned above with existing conformal prediction techniques and other considerations, we claim the desiderata for a trustworthy RAG algorithm as the following: \textbf{A}, the algorithm should provide provable end-to-end guarantees for the RAG system; \unsure{\textbf{B}, the end-to-end guarantee should be on the semantic meanings, instead of specific responses;} \textbf{C}, the algorithm should be sufficiently general to work with different retrievers and LLM, including both black-box API and open-source models; \textbf{D}, the algorithm should provide as higher end-to-end efficiency as possible. 

Overall, we summarize our contributions as follows. First, we apply conformal prediction and global hypothesis testing to provide \textbf{the first end-to-end guarantee} for RAG. Our algorithm can work with LLMs with different API accesses, including black-box and open-source. Second, our algorithm includes a novel way to quantify the uncertainty for each semantic meaning and obtain the first coverage guarantee at the semantic level. Third, we incorporate Bayesian optimization to improve the end-to-end efficiency of the resulting prediction sets. Furthermore, we designed comprehensive experiments to verify TRAG, including \textbf{four} datasets, \textbf{two} different retrievers, \textbf{two} different LLM API accesses, \textbf{two} prompt templates, \textbf{five} coverage levels. We reported both quantitative and qualitative results and analysis. Experiments showed that: \textbf{A}, our end-to-end guarantees hold in different settings; \textbf{B}, incorporating the Bayesian optimization can improve efficiency by \todo{add quantitative results}.
